Numerical study of the overlap Lee-Yang singularities in the three-dimensional Edwards-Anderson model

We have characterized numerically, using the Janus computer, the Lee-Yang complex singularities related to the overlap in the 3D Ising spin glass with binary couplings in a wide range of temperatures (both in the critical and in the spin-glass phase). Studying the behavior of the zeros at the critical point, we have obtained an accurate measurement of the anomalous dimension in very good agreement with the values quoted in the literature. In addition, by studying the density of the zeros we have been able to characterize the phase transition and to investigate the Edwards-Anderson order parameter in the spin-glass phase, finding agreement with the values obtained using more conventional techniques.

==> PaxHeaders.11486/paper_submit.tex <==
30 mtime=1355757775.650736161
30 atime=1355757959.649429335
29 ctime=1355757941.03545954

